Smart, Sparse Contours to Represent and Edit Images

We study the problem of reconstructing an image from information stored at contour locations. We show that high-quality reconstructions with high fidelity to the source image can be obtained from sparse input, e.g., comprising less than $6\%$ of image pixels. This is a significant improvement over existing contour-based reconstruction methods that require much denser input to capture subtle texture information and to ensure image quality. Our model, based on generative adversarial networks, synthesizes texture and details in regions where no input information is provided. The semantic knowledge encoded into our model and the sparsity of the input allows to use contours as an intuitive interface for semantically-aware image manipulation: local edits in contour domain translate to long-range and coherent changes in pixel space. We can perform complex structural changes such as changing facial expression by simple edits of contours. Our experiments demonstrate that humans as well as a face recognition system mostly cannot distinguish between our reconstructions and the source images.

==> background.tex <==
\section{Related Work}
Our paper relates mainly to two research topics: image synthesis and generative models, which will be briefly reviewed in this section.

Image synthesis from spare representations have received much attention.

Talk about:

1. Eldar edge completeness + early vision representation from edge zero crossing
2. PDE based reconstruction from contours (Weichert et. al.).
3. GANs, Pix2Pix and related papers.
4. Image compression.
5. Image editing papers - contour2image editing. Sketch2images etc. 
6. Representation learning: colorization paper of Phillip, context encoder, abhinav gupta blah blah. Can be short or moved to intro.

==> implementation.tex <==
\section{Implementation Details} 
\label{sec:implementation}
Our models were implemented in Tensorflow. We will release our trained models and code. To achieve the editing effects, we built a simple graphical user interface (GUI) that allows editing the contour map using simple operations such as moving, scaling or erasing sets of contours. Note that although the user edits the contour map, the underlying features change in the appropriate manner (for example, if some contours are removed, then the features associated with those contours are also removed). \afterfigure

\paragraph{Computing Input Representation:} Edge probability maps were extracted using   \cite{dollar2013structured} followed by non-maximum suppression as a post processing. The computed maps were binarized by keeping $x$ percentile of edges, where $x$ is the desired percentage of nonzero pixels in the binary edge map. We group the edges into contours and filter out short contours (length less then 10 pixels). Gradients are computed by simple forward differences. \afterfigure
\paragraph{LFN and HFN:}
Both LFN and HFN are ``U-Nets'' \cite{isola2016image}. We adopt the notations in \cite{isola2016image} and denote a convolution layer with $k$ filters followed by batch normalization by $\texttt{Ck}$ for ReLU activation, and $\texttt{Clk}$ for LeakyReLU (slop 0.2). For 256$\times$256 images the number of filters in the encoder  is given by: $\texttt{Cl64-Cl128-Cl256-Cl512-Cl512-Cl512}$, hence the spatial resolution of the bottleneck is $4\times4$. The number of filters in each layer of the decoder is given by: $\texttt{C512-C512-C256-C128-C64-C64}$ (filters in decoder are bigger because of the skip connections). All convolutional filters are size $4 \times 4$, and we use strides of size $2$.\afterfigure

\paragraph{Dilated-Patch Discriminator}
Our discriminator (Fig.~3(c)) is a combination of a ``patch discriminator'' \cite{isola2016image} and a branch of dilated convolution filters. Let $D_{r}k$ denote a dilated convolution with sampling rate $r$, leaky ReLU and $k$ filters. Then our patch discriminator architecture is given by $\texttt{Cl64-Cl128-Cl256}$ followed by $4$ parallel dilated convolutions ${\{\texttt{D}_{2}\texttt{256}, \texttt{D}_{4}\texttt{256}, \texttt{D}_{8}\texttt{256}, \texttt{D}_{12}\texttt{256}}\}$, which are concatenated, and a final convolution layer with a single channel output.

The network used for learning the input representation (see Sec.~4) is similar and consists of a branch of  dilated convolutions, each followed by regular a convolution layer. That is,
{\small ${\{\texttt{D}_{4}\texttt{32}-\texttt{C3}, \texttt{D}_{8}\texttt{256}-\texttt{C3}, \texttt{D}_{12}\texttt{256}-\texttt{C3}, \texttt{D}_{16}\texttt{256}-\texttt{C3}}\}$}, which are added to form the final output.\afterfigure

\paragraph{Training hyper-parameters and details}
For each dataset, LFN and HFN were trained from scratch (weights were  
initialized from a Gaussian distribution with mean 0 and
standard deviation 0.02). We used Adam optimizer with $\beta=0.5, \epsilon=1e^{-4}$, and batch size of $16$ in all training runs except when training on 512$\times$512 where we used size of $8$. We used learning rate of $0.0002$ for the generator, and $0.00002$ for the discriminator, with decay rate of $0.98$ every $10000$ steps. During training we resized the images such that the small dimension is at the desired resolution and then randomly cropped to desired size. The relative weight of the adversarial loss vs. reconstruction loss was 100 in all our experiments.

During the HFN training, the weights of the LFN remained fixed, and we alternate between stepping the discriminator and generator in ratio of 2:1 in favor of the discriminator. When working with learned features, the weights feature network remained fixed during HFN training.

 We trained on the VGG dataset at two spatial resolutions: $256 \times 256$ and $512 \times 512$. For Birds and Dogs, we used the original train/test splits, and for the VGG dataset we filtered out low resolution images from the train and test sets, to avoid reconstruction of JPEG artifacts. The VGG has 30227 samples and was trained for 210 epochs for both LFN and HFN; CUB Birds has 8855 samples and was trained for 720 epochs; Dogs dataset has 12000 training samples and was trained for 500 epochs.

\paragraph{Texture Loss} We use the texture loss in Section 6.1 to evaluate our reconstructions. This loss was defined in \cite{ustyuzhaninov2016does}.


% \section{Implementation Details} 
% \label{sec:implementation}
% Our models were implemented in Tensorflow. We will release our trained models and code. To achieve the editing effects, we built a simple graphical user interface (GUI) that allows editing the contour map using simple operations such as moving, scaling or erasing sets of contours. Note that although the user edits the contour map, the underlying features change in the appropriate manner (for example, if some contours are removed, then the features associated with those contours are also removed). \afterfigure

% \paragraph{Computing Input Representation:} Edge probability maps were extracted using   \cite{dollar2013structured} followed by non-maximum suppression as a post processing. The computed maps were binarized by keeping $x$ percentile of edges, where $x$ is the desired percentage of nonzero pixels in the binary edge map. We group the edges into contours and filter out short contours (length less then 10 pixels). Gradients are computed by simple forward differences. \afterfigure
% \paragraph{LFN and HFN:}
% Both LFN and HFN are ``U-Nets'' \cite{isola2016image}. We adopt the notations in \cite{isola2016image} and denote a convolution layer with $k$ filters followed by batch normalization by $\texttt{Ck}$ for ReLU activation, and $\texttt{Clk}$ for LeakyReLU (slop 0.2). For 256$\times$256 images the number of filters in the encoder  is given by: $\texttt{Cl64-Cl128-Cl256-Cl512-Cl512-Cl512}$, hence the spatial resolution of the bottleneck is $4\times4$. The number of filters in each layer of the decoder is given by: $\texttt{C512-C512-C256-C128-C64-C64}$ (filters in decoder are bigger because of the skip connections). All convolutional filters are size $4 \times 4$, and we use strides of size $2$.\afterfigure

% \paragraph{Dilated-Patch Discriminator}
% Our discriminator (Fig.~\ref{fig:pipeline}(c)) is a combination of a ``patch discriminator'' \cite{isola2016image} and a branch of dilated convolution filters. Let $D_{r}k$ denote a dilated convolution with sampling rate $r$, leaky ReLU and $k$ filters. Then our patch discriminator architecture is given by $\texttt{Cl64-Cl128-Cl256}$ followed by $4$ parallel dilated convolutions ${\{\texttt{D}_{2}\texttt{256}, \texttt{D}_{4}\texttt{256}, \texttt{D}_{8}\texttt{256}, \texttt{D}_{12}\texttt{256}}\}$, which are concatenated, and a final convolution layer with a single channel output.

% The network used for learning the input representation (see Sec~\ref{sec:input_features} is similar and consists of a branch of  dilated convolutions, each followed by regular a convolution layer. That is,
% {\small ${\{\texttt{D}_{4}\texttt{32}-\texttt{C3}, \texttt{D}_{8}\texttt{256}-\texttt{C3}, \texttt{D}_{12}\texttt{256}-\texttt{C3}, \texttt{D}_{16}\texttt{256}-\texttt{C3}}\}$}, which are added to form the final output.\afterfigure

% \paragraph{Training hyper-parameters and details}
% For each dataset, LFN and HFN were trained from scratch (weights were  
% initialized from a Gaussian distribution with mean 0 and
% standard deviation 0.02). We used Adam optimizer with $\beta=0.5, \epsilon=1e^{-4}$, and batch size of $16$ in all training runs except when training on 512$\times$512 where we used size of $8$. We used learning rate of $0.0002$ for the generator, and $0.00002$ for the discriminator, with decay rate of $0.98$ every $10000$ steps. During training we resized the images such that the small dimension is at the desired resolution and then randomly cropped to desired size. The relative weight of the adversarial loss vs. reconstruction loss was 100 in all our experiments.

% During the HFN training, the weights of the LFN remained fixed, and we alternate between stepping the discriminator and generator in ratio of 2:1 in favor of the discriminator. When working with learned features, the weights feature network remained fixed during HFN training.

%  We trained on the VGG dataset at two spatial resolutions: $256 \times 256$ and $512 \times 512$. For Birds and Dogs, we used the original train/test splits, and for the VGG dataset we filtered out low resolution images from the train and test sets, to avoid reconstruction of JPEG artifacts. The VGG has 30227 samples and was trained for 210 epochs for both LFN and HFN; CUB Birds has 8855 samples and was trained for 720 epochs; Dogs dataset has 12000 training samples and was trained for 500 epochs.



